Modeling subjectivity (by Mimicking Annotator Annotation) in toxic comment identification across diverse communities

The prevalence and impact of toxic discussions online have made content moderation crucial.Automated systems can play a vital role in identifying toxicity, and reducing the reliance on human moderation.Nevertheless, identifying toxic comments for diverse communities continues to present challenges that are addressed in this paper.The two-part goal of this study is to(1)identify intuitive variances from annotator disagreement using quantitative analysis and (2)model the subjectivity of these viewpoints.To achieve our goal, we published a new dataset\footnote{\url{https://github.com/XXX}} with expert annotators' annotations and used two other public datasets to identify the subjectivity of toxicity.Then leveraging the Large Language Model(LLM),we evaluate the model's ability to mimic diverse viewpoints on toxicity by varying size of the training data and utilizing same set of annotators as the test set used during model training and a separate set of annotators as the test set.We conclude that subjectivity is evident across all annotator groups, demonstrating the shortcomings of majority-rule voting. Moving forward, subjective annotations should serve as ground truth labels for training models for domains like toxicity in diverse communities.

==> 0.abstract.tex <==
\begin{abstract}

The prevalence and impact of toxic discussions online have made content moderation crucial. Automated systems can play a vital role in identifying toxicity, and reducing the reliance on human moderation. Nevertheless, identifying toxic comments for diverse communities continues to present challenges that are addressed in this paper. The two-part goal of this study is to (1) identify intuitive variances from annotator disagreement using quantitative analysis and (2) model the subjectivity of these viewpoints. To achieve our goal, we published a new dataset\footnote{\url{https://github.com/XXX}} with expert annotators' annotations and used two other public datasets to identify the subjectivity of toxicity. Then leveraging the Large Language Model (LLM), we evaluate the model’s ability to mimic diverse viewpoints on toxicity by varying the size of the training data and utilizing the same set of annotators as the test set used during model training and a separate set of annotators as the test set.  
We conclude that subjectivity is evident across all annotator groups, demonstrating the shortcomings of majority-rule voting. Moving forward, subjective annotations should serve as ground truth labels for training models for domains like toxicity in diverse communities.  





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % It has become crucial to moderate online content due to the prevalence and impact of toxic discussion, especially by using automated systems for identifying toxicity, and alleviating the need for human moderation. 
% % Human-annotated labels are a critical source of ground truth for training models to identify toxic comments.
% % However, a key limiting factor in using toxicity datasets is the low consistency and reliability of annotator labels due to their intrinsic subjectivity.
% % In addition to reducing accuracy, this can drastically impact the fairness of the resulting models, since comments originating from and addressed to minority communities are systematically mislabeled.
% % created using toxic datasets. 
% The prevalence and impact of toxic discussions online have made content moderation crucial. Automated systems can play a vital role in identifying toxicity, and reducing the reliance on human moderation. Nevertheless, identifying toxic comments for diverse communities continues to present challenges that are addressed in the paper.
% % However, effectively identifying toxic comments in diverse communitiescontinues to present challenges that are addressed in this paper.
% % It has become crucial to moderate online content due to the prevalence and impact of toxic discussion, especially by using automated systems for identifying toxicity, and alleviating the need for human moderation. However identifying toxic comments for diverse communities are still challenging.
% % In this paper, we discuss the identification of toxic comments across diverse communities.
% First, we publish a set of annotations by `expert annotators', of potentially toxic comments, along with their rationales\footnote{\url{https://github.com/XXXX}}. 
% % \footnote{https://github.com/google-research-datasets/toxicity-replication}. 
% Then we investigate the subjectivity of toxicity using quantitative analysis to understand the extent and circumstances of disagreement caused by toxicity-related subjectivity.
% % \footnote{https://github.com/google-research-datasets/toxicity-replication/blob/main/toxicity\textunderscore rep \textunderscore dataset.csv}
% % and the potential sources of subjectivity.
%  % We publish a new corpus of 50 comments, manually annotated for the presence and type of toxicity by 10 expert annotators. Using this dataset along with two publicly available dataset we quantitatively and qualitatively analyze the annotations to understand the extent and circumstances of disagreement caused by toxicity-related subjectivity and the potential sources of subjectivity.
% % Then we build on the understanding of subjectivity to present a demonstration within the framework of the Large Language Model (LLM). 
% Building upon our understanding of subjectivity, we proceed to showcase a demonstration within the framework of the Large Language Model (LLM) to evaluate the model's ability to capture different viewpoints on toxicity. To accomplish this goal, we adopt two approaches: varying the size of the training data and utilizing the same set of annotators used during model training and a separate set of annotators as the test set. 
% % This comprehensive approach enables us to comprehensively evaluate and analyze the performance of the model across different training data sizes and diverse annotator perspectives.
% % experiments with respect to different training sizes and different test sets of annotators to assess the model's capability to reproduce different viewpoints on toxicity. 
% % that imitate toxicity annotations from a set of annotators 
% % to assess their capability to reproduce different viewpoints on toxicity. We also test how our published dataset performs when the model is trained with a completely different dataset. 
% % In terms of modeling, we show that it is important to know the training size as well as what set of annotators are used for training and testing in order to understand the model's performance for mimicking annotators.
% % We conclude that rather than using majority voting we need to employ subjective annotations as ground truth labels as well as the need to check the set of annotators for training models and testing in order to identify toxic comments for diverse communities.
% % We conclude that there exist different types of subjectivity depending on different types of annotators. Therefore 
% % We conclude that subjectivity not only exists among non-expert annotators but also among expert annotators and across different groups of annotators. Therefore rather than employing majority-rule voting, subjective annotations should be used as ground truth labels for the model in order to identify toxic remarks for different communities. Understanding the size of the training data and the specific sets of annotators' data used as test sets is crucial when modeling different perspectives of toxicity annotations.
% We conclude that subjectivity is evident across all annotator groups. Therefore, instead of relying on majority-rule voting, subjective annotations should serve as ground truth labels for training models to identify toxic comments in diverse communities. In the case of modeling, it is crucial to consider the training data size and the specific annotator sets used as test sets to better capture various perspectives in toxicity annotations.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% In order to model different perspectives of toxicity annotations it is very important to understand training requirements and testing set of annotators.
% and also (2) understand training size as well as training and testing set of annotators in order to understand model's performance in mimicking annotators.

% we need to understand requirements for training models which can be tailored to those communities.

 % in order to show that the model must take into account each different type of annotator's point of view while identifying toxicity.
 
 % using two different ways : with soft-tuning and without soft-tuning. LLM takes into account 
 % Finally we discuss the implications of our strategies in all other subjective data sets.
% by taking into account the subjectivity of each annotator for toxic comments
 
 % Finally we discuss possible approaches to address subjective dataset with a better knowledge of inherent subjectivity as well as some potential suggestions to improve model's performance for subjective datasets.
 
 % we assess performance of LLM imitating each annotator's subjectivity of toxic annotation using two different ways: with soft tuning and without soft tuning 


 % We thereafter show the output of large language model (LLM) on imitating annotator's subjectivity for toxic comments using two different ways: with soft tuning and without soft-tuning.
 % such that the model can represent diverse communities of annotators while trained on annotation from raters of varied communities.
  

 
 
 % train large language model (LLM) using each annotator's toxicity annotation  to model subjectivity of each annotator to reflect diverse communities.

 



% imitating annotator's subjectivity for toxic comments. 

 
 % the subjectivity of toxic dataset by mimicking the subjectivity of each rater using large language model. 


% Online platforms have become an essential medium of discussion on a global scale.
% Due to the prevalence and impact of toxic discussions, it has become crucial to reduce toxicity and harassment on these platforms. 
% However, reducing toxicity is still a challenging problem due to the lack of understanding of the varied but valid opinions of human annotators for toxicity. 

% inside each group of annotators and across two pool of annotators to understand the extent and circumstances of inter-rater disagreement caused by toxicity-related subjectivity. In addition to that, we qualitatively analyze the rationale provided by expert annotators to understand the sources of subjectivity. Quantitative analysis reveals that there is a considerable amount of disagreement not only among non-expert annotators but also among expert annotators. The results from the sources of subjectivity illustrate the potential sources of agreement and disagreement between expert annotators. This suggests that each expert rater adds a unique kind of subjectivity when annotating comments relating to toxicity. 
% Therefore we verify the suggestion by mimicking the subjectivity of each rater using large language model. 
% Finally, we discuss the potential ways to address toxicity as well as other subjective datasets with a better understanding of their inherent subjectivity. 

% \textcolor{red}{Disclaimer: This paper contains comments that are offensive by nature.}

\end{abstract}
